Robust Data Watermarking in Language Models by Injecting Fictitious Knowledge

Data watermarking in language models injects traceable signals, such as specific token sequences or stylistic patterns, into copyrighted text, allowing copyright holders to track and verify training data ownership. Previous data watermarking techniques primarily focus on effective memorization during pretraining, while overlooking challenges that arise in other stages of the LLM lifecycle, such as the risk of watermark filtering during data preprocessing and verification difficulties due to API-only access. To address these challenges, we propose a novel data watermarking approach that injects plausible yet fictitious knowledge into training data using generated passages describing a fictitious entity and its associated attributes. Our watermarks are designed to be memorized by the LLM through seamlessly integrating in its training data, making them harder to detect lexically during preprocessing. We demonstrate that our watermarks can be effectively memorized by LLMs, and that increasing our watermarks' density, length, and diversity of attributes strengthens their memorization. We further show that our watermarks remain effective after continual pretraining and supervised finetuning. Finally, we show that our data watermarks can be evaluated even under API-only access via question answering.

==> related.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Membership inference} Membership inference techniques are used to infer which data are members of the training data \cite{hu_membership_2022}. 
Since neural models can overfit to their training data, the model's loss on training examples often carries signals about whether a given example was used for training \cite{DBLP:conf/sp/ShokriSSS17, shi2023detecting}. Recently, traditional membership inference techniques on LLMs have been shown to be largely ineffective, as they do not memorize individual occurrences due to their large data, large batch size training regime \cite{duan2024membership}. 

To overcome these limitations, membership inference techniques have pursued alternative strategies which can strengthen the detection. For one, there is a practical need to infer membership about a dataset rather than single examples, and this setting allows membership information to be accumulated across examples \cite{oren2023proving, maini2024llm}. Another practical affordance is that data creators or copyright holders often distribute their data, so they can watermark it before public release \cite{Wei2024ProvingMI, Meeus2024CopyrightTF, zhang2024membershipinferenceattacksprove}. Detecting watermarks rather than the data itself greatly enhance the membership effectiveness and can contain the randomness necessary to achieve statistical guarantees.

\paragraph{Data watermarking} To watermark the data for purposes of membership inference, the literature has previously explored: \textit{(a) Random sequences.} \citet{Wei2024ProvingMI} appends randomly generated sequences, such as SHA hashes, to the end of a document as a watermark. To cause memorization, such watermarks need to be duplicated across documents exactly. \textit{(b) Random word sequences.} \citet{Meeus2024CopyrightTF} proposes ``copyright traps'' which randomly sampled word sequences and inserts them into documents. These sequences are repeated across documents to increase the likelihood of memorization and detection.

All existing methods use exact duplication of these watermarks to cause memorization. These randomly generated watermarks are often highly distinct and unusual and they can be filtered by a determined adversary. \citet{Shilov2024MosaicMF} has recognized duplication as a major weakness of these watermarks and introduce ``fuzzy'' copyright traps which can evade simple deduplication filters by introducing slight variations so that each instance of a copyright trap is unique while still being memorized by the model for later detection.

\paragraph{LLM knowledge acquisition} Many studies have documented the ability of language models to memorize vast amounts of factual information during pretraining \cite[inter alia]{petroni-etal-2019-language, AllenZhu2023PhysicsOL}. The repeated exposure to a fact in diverse forms plays an important role in the retention and usability of that fact for an LLM  \cite{chang2024largelanguagemodelsacquire}, and \citet{kandpal_large_2023} show that very large LLMs can memorize even long tail knowledge. Our approach using fictitious knowledge as watermarks leverages the model's ability to store underlying factual knowledge and we insert varied surface forms of a fact to better evade filters, which makes the watermark more resilient against detection and removal.

After pretraining, instruction tuning or other post-training techniques can cause degradation on NLP tasks, often termed an ``alignment tax'' \cite{ouyang2022traininglanguagemodelsfollow}. \citet{chen2024continualmemorizationfactoidslarge} study the degradation of factoid memorization after post-training, and one incidental finding is that the memorization of random strings degrade more than natural language facts after post-training. Other data watermarking works only study memorization of pretraining, and  we are the first to study the retention of data watermarks after post-training, another practical gap to close when applying data watermarks. Post-training is commonly used in training state of the art LLMs \cite[i.e.,][]{grattafiori2024llama3herdmodels} and fictitious knowledge provides provide another advantage in memorization.
